Online Resource Allocation under Horizon Uncertainty

We study stochastic online resource allocation: a decision maker needs to allocate limited resources to stochastically-generated sequentially-arriving requests in order to maximize reward. At each time step, requests are drawn independently from a distribution that is unknown to the decision maker. Online resource allocation and its special cases have been studied extensively in the past, but prior results crucially and universally rely on the strong assumption that the total number of requests (the horizon) is known to the decision maker in advance. In many applications, such as revenue management and online advertising, the number of requests can vary widely because of fluctuations in demand or user traffic intensity. In this work, we develop online algorithms that are robust to horizon uncertainty. In sharp contrast to the known-horizon setting, no algorithm can achieve even a constant asymptotic competitive ratio that is independent of the horizon uncertainty. We introduce a novel generalization of dual mirror descent which allows the decision maker to specify a schedule of time-varying target consumption rates, and prove corresponding performance guarantees. We go on to give a fast algorithm for computing a schedule of target consumption rates that leads to near-optimal performance in the unknown-horizon setting. In particular, our competitive ratio attains the optimal rate of growth (up to logarithmic factors) as the horizon uncertainty grows large. Finally, we also provide a way to incorporate machine-learned predictions about the horizon which interpolates between the known and unknown horizon settings.

==> distribution.tex <==
\section{Known Distribution and Sample Access}

In this section, we make the environment less adversarial and assume that there is an underlying distribution $\T$ supported on $[\tau_1, \tau_2]$ from which the horizon $T$ is drawn. The decision maker does not know the exact value of $T$ and wishes the maximize the expected performance ratio
\begin{align*}
	e(A) = \inf_{\PP} \E_{T \sim \T}[ c(A|T, \PP) ] = \inf_{\PP} \E_{T \sim \T} \left[ \frac{\E_{\vec\gamma \sim \PP^T}\left[R(A|T, \vec \gamma) \right]}{\E_{\vec\gamma \sim \PP^T}\left[\opt(T, \vec\gamma)\right]} \right]
\end{align*}

We consider two information environments: (i) The decision-maker knows the distribution $\T$; and (ii) The decision maker has access to $n$ samples from $\T$.

\subsection{Upper Bound on the Expected Performance Ratio}

We begin by showing that, in the worst case, we do not gain anything from the knowledge of the distribution of the horizon. In particular, we show that there exists a distribution $\T$ such that the knowledge of $\T$ confers no benefit and the optimal course of action is to ignore $\T$ and maximize the competitive ratio. This yields the same upper bound on the competitive ratio as we had in Theorem~\ref{thm:upper-bound}. In fact, we prove it by exploiting the fact that the worst-case request distribution used to prove Theorem~\ref{thm:upper-bound} consisted of a concave reward and linear consumption function, which ensures strong duality and allows us to construct the worst-case horizon distribution using the dual variables. 

In the remainder of this subsection, we will employ the notation introduced in Subsection~\ref{sec:upper-bound}. Set the number of resources to $m = 1$ and $B = \tau_2$ (which implies $\rho_{\tau_2} = 1$). Moreover, define the singleton request space $\S_r = \{(f_r, I, \X)\}$ for a parameter $r \in (0, 1]$, where $\X = [0,\tau_2/\tau_1]$, and $f_r(x) = x^r$, $I(x) = x$ for all $x \in \X$. Note that $f_r$ is concave for all $r \in (0,1)$. Let $\PP_r$ be the canonical distribution on $\S_r$ that serves the request $(f_r, I, \X)$ with probability one. Since all requests are identical, we abuse notation and use $\opt(T, r)$ (similarly $R(A|T, r)$) to denote the hindsight-optimal reward $\opt(T, \vec\gamma)$ (total reward $R(A|T, \vec\gamma)$ of algorithm $A$) when $\vec \gamma \sim \PP_r^T$, i.e., $\gamma_t = (f_r, I, \X)$ for all $t \leq T$. Moreover, as argued in Subsection~\ref{sec:upper-bound}, we can focus on deterministic online algorithms without loss of generality.

\begin{proposition}\label{prop:dist-upper-bound}
	For every $r \in (0,1)$, there exists a distribution $\T_r$ of the horizon $T$ such that 
	\begin{align*}
		\sup_A \E_{T \sim \T_r} \left[ \frac{R(A|T,r)}{\opt(T,r)} \right] = \sup_A \min_{T \in [\tau_1, \tau_2]} \frac{R(A|T,r)}{\opt(T,r)}
	\end{align*}
	where $\sup_A$ denotes the supremum over all online algorithms $A$ with the knowledge of the horizon distribution $\T_r$ and the request distribution $\PP_r$. 
\end{proposition}

\begin{proof}
	Fix $r \in (0,1)$. We begin by showing that for all $r \in (0,1)$, we have
	\begin{align*}
		\sup_A \min_{T \in [\tau_1, \tau_2]} \frac{R(A|T,r)}{\opt(T,r)} \quad = \quad \max \quad &z\\
		\text{s.t.} \quad &z \leq \frac{\sum_{t=1}^T f_r(x_t)}{\opt(T,r)} &\forall T \in [\tau_1, \tau_2]\\
		&\sum_{t=1}^{\tau_2} x_t \leq B\\
		&0 \leq x_t \leq \tau_2/\tau_1 &\forall x \in [\tau_2]
	\end{align*}
	The RHS is a convex program because $f_r$ is concave. Let $A$ be any online algorithm. Let $x(A)_t$ denote the action taken by $A$ at time $t$. Then, $x_t = x(A)_t$ and
	\begin{align*}
		z = \min_{T \in [\tau_1, \tau_2]} 	\frac{\sum_{t=1}^T f_r(x(A)_t)}{\opt(T,r)} = \min_{T \in [\tau_1, \tau_2]}  \frac{R(A|T,r)}{\opt(T,r)}\,
	\end{align*}
	is a feasible solution of the convex program, thereby establishing the `$\leq$' direction. The other direction is equally straightforward: Any feasible solution $(x_t, z)$ of the convex program naturally gives rise to an algorithm which takes action $x_t$ at time $t$.
	
	Note that $x_t = 1/2$ and $z = 0$ is a feasible solution of the convex program that satisfies
	\begin{align*}
		z < \frac{\sum_{t=1}^T f_r(x_t)}{\opt(T,r)} \quad \forall T \in [\tau_1, \tau_2]
	\end{align*}
	Therefore, by Slater's rule (see \citealt{}), we get that strong duality holds and there exists an optimal dual multiplier $\{p_T\}_{T=\tau_1}^{\tau_2}$ such that $p_T \geq 0$ for all $T \in [\tau_1, \tau_2]$ and
	\begin{align*}
		\sup_A \min_{T \in [\tau_1, \tau_2]} \frac{R(A|T,r)}{\opt(T,r)} \quad = \quad \max \quad & z + \sum_{T=\tau_1}^{\tau_2} p_T \left( \frac{\sum_{t=1}^T f_r(x_t)}{\opt(T,r)} - z\right) \\
		\text{s.t.} \quad &\sum_{t=1}^{\tau_2} x_t \leq B\\
		&0 \leq x_t \leq \tau_2/\tau_1 &\forall x \in [\tau_2]\\
		= \quad \max \quad & z\left( 1 - \sum_{T=\tau_1}^{\tau_2} p_T \right) + \sum_{T=\tau_1}^{\tau_2} p_T \cdot\frac{\sum_{t=1}^T f_r(x_t)}{\opt(T,r)} \\
		\text{s.t.} \quad &\sum_{t=1}^{\tau_2} x_t \leq B\\
		&0 \leq x_t \leq \tau_2/\tau_1 &\forall x \in [\tau_2]
	\end{align*}
	Observe that, since $z$ is an unrestricted variable, we need $\sum_{T=\tau_1}^{\tau_2} p_T =1$ to ensure that the restated (Lagrangian) optimization problem is bounded, which is necessary because the LHS is bounded. Hence, we get
	\begin{align*}
		\sup_A \min_{T \in [\tau_1, \tau_2]} \frac{R(A|T,r)}{\opt(T,r)} \quad
		= \quad \max \quad & \sum_{T=\tau_1}^{\tau_2} p_T \cdot\frac{\sum_{t=1}^T f_r(x_t)}{\opt(T,r)} \\
		\text{s.t.} \quad &\sum_{t=1}^{\tau_2} x_t \leq B\\
		&0 \leq x_t \leq \tau_2/\tau_1 &\forall x \in [\tau_2]
	\end{align*}
	Let $\T_r$ be the distribution which picks horizon $T$ with probability $p_T$ for all $T \in [\tau_1, \tau_2]$. Then, once again, we can use the equivalence between feasible solutions of the convex program and the actions of an online algorithm ($x_t = x(A)_t$) to get
	\begin{align*}
		\sup_A \min_{T \in [\tau_1, \tau_2]} \frac{R(A|T,r)}{\opt(T,r)} \quad
		= \quad \max \quad & \sum_{T=\tau_1}^{\tau_2} p_T \cdot\frac{\sum_{t=1}^T f_r(x_t)}{\opt(T,r)} \quad = \quad \sup_A \E_{T \sim \T_r} \left[ \frac{R(A|T,r)}{\opt(T,r)} \right]  \\
		\text{s.t.} \quad &\sum_{t=1}^{\tau_2} x_t \leq B\\
		&0 \leq x_t \leq \tau_2/\tau_1 \quad \forall x \in [\tau_2]
	\end{align*}
	as required.
\end{proof}

Combining Proposition~\ref{prop:dist-upper-bound} and Theorem~\ref{thm:upper-bound} immediately yields the following corollary.

\begin{corollary}\label{cor:dist-upper-bound}
    For all $r \in (0,1)$ and $1 \leq \tau_1 \leq \tau_2$, there exists a horizon distribution $\T_r$ such that every online algorithm $A$ with knowledge of $\T_r$ satisfies
    \begin{align*}
        \E_{T \sim \T_r} \left[ \frac{R(A|T,r)}{\opt(T,r)} \right] \leq \frac{1}{\left(1 + (1 - r)^{1/r} \cdot \ln(\tau_2/\tau_1) + \ln\left( \frac{\tau_1}{\tau_1 + 1} \right) \right)^r}\,. 
    \end{align*}
	In particular, for $r = 1 - \{1/\ln\ln(\tau_2/\tau_1)\}$, $\tau_2/\tau_1 > e^e$ and $\tau_1 \geq 1$, we have
	\begin{align*}
		\E_{T \sim \T_r} \left[ \frac{R(A|T,r)}{\opt(T,r)} \right] \leq  \frac{e\cdot \ln\ln(\tau_2/\tau_1)}{\ln(\tau_2/\tau_1)}\,.
	\end{align*}
	The above bounds hold even for online algorithms that have prior knowledge of $\PP_r$ before time $t=1$.
\end{corollary}

Even though the aforementioned results state that the knowledge of the horizon distribution $\T$ does not improve performance in the worst case, reality is seldom worst case and it is worth developing algorithms for this setting. We do so next, starting with the case of the known horizon and then moving onto sample access.

\subsection{Optimizing the Target Sequence for Known Distribution}

For this subsection, assume that the horizon distribution $\T$ is known to the decision maker. Let $A$ denote Algorithm~\ref{alg:dual-descent} with target consumption sequence $\vec\lambda$. Then, Proposition~\ref{prop:master} implies that the expected performance ratio satisfies:
\begin{align*}
	e(A) = \inf_{\PP} \E_{T \sim \T}[ c(A|T, \PP) ] \geq \inf_{\PP} \E_{T \sim \T}[ \inf_{\PP} c(A|T, \PP) ] = \E_{T \sim \T}[ c(\vec\lambda, T)] - \epsilon
\end{align*}
Thus, we would like to find the target consumption sequence which maximizes $\E_{T \sim \T}[ c(\vec\lambda, T)]$, which is what we do next.

\begin{proposition}\label{prop:known-dist-LP}
	For budget $B$, uncertainty window $[\tau_1, \tau_2]$ and horizon distribution $\T$ which picks horizon $T$ with probability $p_T$, we have
	\begin{align*}
		\max_{\vec\lambda} \E_{T \sim \T}[ c(\vec\lambda, T) ] \quad  = \quad  \max \quad & \sum_{T = \tau_1}^{\tau_2} p_T \cdot \frac{\sum_{t=1}^T y_t}{T} \\
		\text{s.t.} \quad
		&y_t \leq \frac{\lambda_{t,j}}{\rho_{T,j}} &\forall j \in [m], t \in [\tau_2]\\
		&y_t \leq 1 &\forall t \in [\tau_2]\\
		&\sum_{t=1}^{\tau_2} \lambda_t \leq B\\
		&\lambda \geq 0
	\end{align*} 
\end{proposition}

Like the Uncertainty Window setting discussed in the previous section, Proposition~\ref{prop:known-dist-LP} allows for efficient computation of the target consumption sequence using an LP. Next, we show how to optimize the target consumption sequence if one does not known the horizon distribution $\T$ but only has sample access to it.

\subsection{Sample Access}













==> fluid.tex <==
\section{Fluid Upper Bound Benchmark}

\begin{algorithm}[t!]
	\SetAlgoLined
	{\bf Input:} Initial dual solution $\mu_1$, initial resource endowment $B_1 = B$, horizon distribution $\T = \{S_t\}_{t=1}^{\tau_2}$, reference function $h: \R^m \rightarrow \R$, and step-size $\eta$. \\
	\For{$t=1,\ldots,T$}{
		Receive request $(f_t, b_t, \X_t) \sim \PP$.\\
		Make the primal decision $x_t$ and update the remaining resources $B_t$:
		\begin{align}
		\tilde{x}_{t} &\in \argmax_{x\in\X_t}\left\{f_{t}(x)-\mu_{t}^{\top} b_{t}(x)\right\} \ ,\label{eq:primal_decision} \\
		x_{t}&=\left\{\begin{array}{cl}
		\tilde{x}_t    & \text{  if } b_t(\tilde{x}_t)\le B_t  \\
		0
		& \text{ otherwise}
		\end{array} \right. \ , \nonumber \\
% 		a_t &= \arg\max_{a\le \rho}\{r(a)+\mu_t^\top a\}\ , \nonumber \\
		B_{t+1} &= B_t - b_t(x_t) . \nonumber
		\end{align}\\
		%   \begin{align*}
		%       \begin{split}
		%           x_{t} &= \tilde{x}_t \text{  if  b_{t}x_{t}\le B_t} \\
		%           &=
		%       \end{split}
		%   \end{align*}
		\textbf{Modified step}: $g_t = S_t\{\rho_{T^*} -b_t(\tilde x_t)\}$.
		
		
		Update the dual variable by mirror descent:
           $\mu_{t+1} = \arg\min_{\mu\in\R_+^m} g_t^\top \mu + \frac{1}{\eta} V_h(\mu, \mu_t)$,
       {\color{black} where $V_h(x,y)=h(x)-h(y)-\nabla h(y)^\top (x-y)$ is the Bregman divergence.}
		
%		\begin{equation}\label{eq:dual_update}
%		       \mu_{t+1} = \arg\min_{\mu\in\cD} \langle -b_t\tx_t, \mu \rangle + \frac{1}{\eta} V_h(\mu, \mu_t) +r^*(-\mu)\ .
%		  \end{equation}
	}
	\caption{Variable Target Dual Mirror Descent Algorithm}
	\label{alg:dist-dual-descent}
\end{algorithm}


In this section, we will assume that the distribution $\T$ over the horizon (supported on $[\tau_1,\tau_2]$ and independent of $\PP$) is known to the decision maker. In particular, let $S_t = P(T \geq t)$ and assume that $\{S_t\}_{t=1}^{\tau_2}$ is known to the decision maker. Set $T^* = E[T] = \sum_{t=1}^{\tau_2} S_t$ (Here, we have used $E[X] = \sum_{x=1}^{\infty} P(X \geq x)$ for every random variable $X$ supported on the positive integers). Consider the following fluid relaxation of the problem
\begin{align*}
	F(\T, \PP) = \max \quad & \sum_{t=1}^{\tau_2} S_t \cdot \E_{\gamma_t \sim \PP}\left[ f_t(x_t(\gamma_t)) \right]\\
	\text{s.t.} \quad &\sum_{t=1}^{\tau_2} \E_{\gamma_t \sim \PP} 	[b_t(x_t(\gamma_t))] \leq B\\
	&x_t: \S \to \X
\end{align*}

Then, the dual of the fluid relaxation is given by
\begin{align*}
	D(\mu| \T, \PP) &=  \mu^T B + \sum_{t=1}^{\tau_2} \max_{x_t:\S \to \X} \E_{\gamma_t \sim \PP}\left[ S_t f_t(x_t(\gamma)) - \mu^T b_t(x_t(\gamma_t)) \right]\\
	&=  \mu^T B \cdot \frac{\sum_{t=1}^{\tau_2} S_t}{E[T]} + \sum_{t=1}^{\tau_2} S_t \max_{{x_t:\S \to \X}} \E_{\gamma_t \sim \PP}\left[ f_t(x_t(\gamma)) - \mu^T b_t(x_t(\gamma_t)) \right]\\
	&=  \sum_{t=1}^{\tau_2} S_t \mu^T \rho_{T^*}  + \sum_{t=1}^{\tau_2} S_t \max_{{x_t:\S \to \X}} \E_{\gamma_t \sim \PP}\left[ f_t(x_t(\gamma)) - \mu^T b_t(x_t(\gamma_t)) \right]\\
	&=  \sum_{t=1}^{\tau_2} S_t \left\{  \E_{\gamma_t \sim \PP}\left[ \max_{x_t \in \X} f_t(x_t) - \mu^T b_t(x_t) \right] + \mu^T \rho_{T^*} \right\}
\end{align*}

We use $\tilde D(\mu|\T, \PP) =  \E_{\gamma_t \sim \PP}\left[ \max_{x_t \in \X} f_t(x_t(\gamma)) - \mu^T b_t(x_t(\gamma_t)) \right] + \mu^T \rho_{T^*}$. Therefore,
\begin{align*}
	D(\mu| \T, \PP) = \left(\sum_{t=1}^{\tau_2} S_t \right) \tilde D(\mu|\T,\PP)  = T^* \cdot \tilde D(\mu|\T,\PP)
\end{align*}




Algorithm~\ref{alg:dist-dual-descent} is a variant of the dual descent algorithm (modification from vanilla dual descent is in the linear loss used for dual descent).




\begin{theorem} Consider Algorithm \ref{alg:dist-dual-descent} with initial dual solution $\mu_1$, initial resource endowment $B_1 = B$, horizon distribution $\T = \{S_t\}_{t=1}^{\tau_2}$, reference function $h(\cdot): \R^m \rightarrow \R$, and step-size $\eta$. For any $T \geq 1$, we have
		\begin{align}\label{eq:master}
			F(\T, \PP) - \E_{T \sim \T, \vec\gamma \sim \PP^{\tau_2}} \left[R(A|T, \vec\gamma)\right] \le C_1 + C_2 \eta \tau_2 + \frac {C_3}{\eta} \,.
		\end{align}
		where $C_1 = \bar f \bar b  / \underline \rho_{T^*}$, $C_2 = (\bar b + \bar \lambda)^2/2\sigma$, $C_3= \max \left\{  V_h(\mu, \mu_1) : \mu \in \{0, (\bar f/\underline \rho_{T^*}) e_1,\ldots, (\bar f/\underline \rho_{T^*}) e_m\}  \right\}$. Here $e_j\in\R^m$ is the $j$-th unit vector and $\underline \rho_{T^*} = \min_j \rho_{T^*,j}$.
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:regret}]

	We split the proof into four steps: (1) The first step involves lower bounding the performance of our algorithm in terms of single-period duals and the complementary slackness term; (2) The second step involves bounding the complementary slackness term using standard regret analysis of mirror descent; (3) The third step involves bounding the optimal from above using the single-period duals; (4) The final step puts it all it all together.
	
	\paragraph{Step 1: Lower bound on algorithm's reward.} Consider the filtration $\mathcal{F} = \{\sigma(\xi_t)\}_t$, where $\xi_t = \{\gamma_1, \dots, \gamma_t\}$ the set of all requests seen till time $t$ and $\sigma(\xi_t)$ is the sigma algebra generated by it. Note that Algorithm~\ref{alg:dist-dual-descent} only collects rewards when there are enough resources left. Let $\tA$ be first time less than $\tau_2$ for which there exists a resource $j$ such that $\sum_{t=1}^{\tA} b_{t,j}(x_t) + \bar{b} \ge B_j$. Here, $\tA = \tau_2$ if this inequality is never satisfied. Observe that $\tA$ is a stopping time w.r.t. $\mathcal{F}$ and it is defined so that we cannot violate the resource constraints before $\tA$. In particular, $x_t = \tilde{x}_t$ for all $t \leq \tA$. Therefore, we get
		\begin{align*}
			f_t(x_t) = f^*(\mu_t) + \mu_t^\top b_t(x_t)
		\end{align*}
		Observe that $\mu_t$ is measurable w.r.t. $\sigma(\xi_{t-1})$ and $\gamma_t$ is independent of $\sigma(\xi_{t-1})$, which allows us to take conditional expectation w.r.t. $\sigma(\xi_{t-1})$ to write
		\begin{align}\label{eq:bound-one-period}
			\mathbb E\left[S_t f_t(x_t)  | \sigma(\xi_{t-1}) \right] \nonumber
			&= S_t \cdot \left\{ \E_{\gamma_t \sim \PP}\left[f^*(\mu_t)\right] + \mu_t^{\top} \rho_{T^*} + \mu_t^\top \left( \E\left[ b_t(x_t)| \sigma(\xi_{t-1}) \right] - \rho_{T^*} \right) \right\}    \nonumber\\
			&=  S_t \cdot \tilde D(\mu_t| \T, \PP) - \mathbb E\left[S_t \cdot \mu_t^\top \left( \rho_{T^*} - b_t(x_t) \right) | \sigma(\xi_{t-1}) \right]
		\end{align}
		where the second equality follows the definition of the single-period dual function.
		
		Define $Z_t = \sum_{s=1}^t S_s \cdot  \mu_s^\top \left(\rho_{T^*} - b_{s} (x_s)\right) - \mathbb E\left[S_s \cdot \mu_s^\top \left(\rho_{T^*} - b_{s} (x_s) \right) | \sigma(\xi_{s-1}) \right]$. Then, $\{Z_t\}_t$ is a martingale w.r.t. the filtration $\mathcal{F}$ because $Z_t \in \sigma(\xi_t)$ and $\E[Z_{t+1} | \sigma(\xi_t)] = Z_t$. As $\tA$ is a bounded stopping time w.r.t. $\mathcal{F}$, the Optional Stopping Theorem yields $\E\left[Z_{\tA}\right] = 0$. Therefore,
		\begin{align*}
			\E\left[\sum_{t=1}^{{\tA}} S_t \cdot \mu_t^\top \left(\lambda_t - b_t(x_t)\right) \right]
			= \E\left[\sum_{t=1}^{{\tA}} \mathbb E\left[S_t\cdot  \mu_t^\top \left(\lambda_t - b_t(x_t)\right) | \sigma(\xi_{t-1}) \right] \right]\,.
		\end{align*}
		A similar argument yields
		\begin{align*}
			\E\left[\sum_{t=1}^{{\tA}} S_t f_t(x_t) \right]
			= \E\left[\sum_{t=1}^{{\tA}} \mathbb E\left[ S_t f_t(x_t) | \sigma(\xi_{t-1}) \right] \right]\,.
		\end{align*}
		Hence, summing over \eqref{eq:bound-one-period} and taking expectations, we get
		\begin{align}\label{eq:alg-lower-bound}
			\mathbb E\left[ \sum_{t=1}^{\tA} S_t f_t(x_t)  \right]
			&=
			\mathbb E\left[ \sum_{t=1}^{\tA} S_t \tilde D(\mu_t| \T, \PP) \right ]  - \mathbb E\left[ \sum_{t=1}^{\tA} S_t \cdot \mu_t^\top \left(   \rho_{T^*} - b_t(x_t) \right) \right] \nonumber\\
			&=
			\mathbb E\left[ \sum_{t=1}^{\tA} S_t \cdot \sum_{t=1}^{\tA} \frac{S_t}{\sum_{s=1}^{\tA} S_s} \cdot \tilde D\left(\mu_t|  \T, \PP \right) \right ]  - \mathbb E\left[ \sum_{t=1}^{\tA} S_t \cdot \mu_t^\top \left(  \rho_{T^*} - b_t(x_t) \right) \right] \nonumber\\
			&\ge
			\mathbb E\left[ \sum_{t=1}^{\tA} S_t \cdot \tilde D\left(\bar\mu_{\tA}|  \T, \PP \right) \right ] - \mathbb E\left[ \sum_{t=1}^{\tA} S_t \cdot \mu_t^\top \left( \rho_{T^*} - b_t(x_t) \right) \right]\,
		\end{align}
	where
	\begin{align*}
		\bar\mu_{\tA} = \sum_{t=1}^{\tA} \frac{S_t \cdot \mu_t}{\sum_{s=1}^{\tA}S_t}.
	\end{align*}
	The inequality follows from the convexity of the single-period dual function. Finally, note that
	\begin{align*}
		\E_{T \sim \T, \vec\gamma \sim \PP^{\tau_2}} \left[R(A|T, \vec\gamma)\right] = \E_{\vec\gamma \sim \PP^{\tau_2}}\left[ \E_T \left[ \sum_{t=1}^{T \wedge \tA} f_t(x_t)  \right] \right] = \E\left[ \sum_{t=1}^\tA S_t f_t(x_t) \right]
	\end{align*}
	
	\paragraph{Step 2: Complementary slackness.} Define $w_t(\mu) \coloneqq \mu^\top(S_t \{\rho_{T^*} - b_t(x_t)\})$. Then, Algorithm~\ref{alg:dual-descent} can be seen as running online mirror descent on the choice of the dual variables with linear losses $\{w_t(\cdot)\}_t$. The gradients of these loss functions are given by $\nabla w_t(\mu) = S_t \{\rho_{T^*} - b_t(x_t)\}$, which satisfy $\|\nabla w_t(\mu)\|_\infty \leq \|b_t(x_t)\|_\infty + \|\lambda(t)\|_\infty \leq \bar b + \bar \lambda$. Therefore, Proposition 5 of \citet{balseiro2020best} implies that for all $\mu \in \R_+^m$:
	\begin{align}\label{eq:regret-omd}
		\sum_{t=1}^{\tA} w_t(\mu_t) - w_t(\mu) \le E(\tA, \mu) \le E(\tau_2,\mu)\,,
	\end{align}
	where $E(t,\mu) = \frac 1 {2\sigma} (\bar{b} + \bar\lambda)^2 \eta \cdot t + \frac{1}{\eta} V_h(\mu,\mu_1)$ is the regret bound of the online mirror descent algorithm after $t$ iterations, and the second inequality follows because $\tA \le \tau_2$ and the error term $E(t,\mu)$ is increasing in $t$.
	
	\paragraph{Step 3: Upper bound on the optimal reward.} For every $\tA \in [1, \tau_2]$, we have
		\begin{align}\label{eq:opt-upper-bound}
			&F(\T, \PP) \nonumber\\
			= &  \frac{\sum_{s=1}^{\tau_2} S_s}{\E[T]} \cdot F(\T, \PP) \nonumber\\
			= &  \frac{\sum_{s=1}^{\tA} S_s}{T^*} \cdot F(\T, \PP) + \frac{\sum_{s=\tA + 1}^{\tau_2}S_s}{T^*} \cdot F(\T, \PP) \nonumber\\
			\leq &  \sum_{s=1}^{\tA} S_s \cdot \frac{D(\bar\mu_{\tA}|\T,\PP)}{T^*} + \sum_{s=\tA + 1}^{\tau_2}S_s \cdot \bar f &\left(F(\T, \PP) \leq T^* \cdot \bar f, \text{weak duality} \right) \nonumber\\
			= &  \sum_{t=1}^{\tA} S_t \cdot \tilde D\left(\bar\mu_{\tA}|  \T, \PP \right)  +  \sum_{t=\tA + 1}^{\tau_2}S_t \cdot \bar f
		\end{align} 
	
	
	\paragraph{Step 4: Putting it all together.} Combining the results from steps 1-3 yields:
	\begin{align*}
		&F(\T, \PP) - \E_{T \sim \T, \vec\gamma \sim \PP^{\tau_2}} \left[R(A|T, \vec\gamma)\right]\\
		\leq\ &  \E_{\vec\gamma \sim \PP^{\tau_2}} \left[ F(\T,\PP) - \sum_{t=1}^{\tA} S_t\cdot \tilde D\left(\bar\mu_{\tA}|  T^*, \PP \right) + \sum_{t=1}^{\tA} S_t \cdot\mu_t^\top \left( \lambda_t - b_t(x_t) \right)\right] & (\text{Equation \ref{eq:alg-lower-bound}})\\
		\leq\ &  \E_{\vec\gamma \sim \PP^{\tau_2}} \left[ \sum_{t=\tA + 1}^{\tau_2} S_t \cdot \bar f + \sum_{t=1}^{\tA} w_t(\mu_t)\right] & (\text{Equation \ref{eq:opt-upper-bound}})\\
		\leq\ &  \underbrace{\E_{\vec\gamma \sim \PP^{\tau_2}} \left[ \sum_{t=\tA + 1}^{\tau_2} S_t \cdot \bar f + \sum_{t=1}^{\tA} w_t(\mu) + E(\tau_2, \mu)\right]}_{\clubsuit} & (\text{Equation \ref{eq:regret-omd}})
	\end{align*}
	for all $\mu \in \R_+^m$. All that remains to complete the proof is choosing the right $\mu$. If $\tA = \tau_2$ (no resource was completely depleted), set $\mu = 0$. If $\tA < \tau_2$, then there exists a resource $j \in [m]$ that nearly got depleted, i.e., $\sum_{t=1}^{\tA} b_{t,j}(x_t) + \bar{b} \ge B_j = T^* \cdot \rho_{T^*}$. Thus, $\sum_{t=1}^{\tA} b_{t,j}(x_t)) \geq - \bar b +  T^* \rho_{T^*,j}$. Therefore, setting $\mu = (\bar f/ \underline \rho_{T^*,j}) e_j$, where $e_j \in \R_m$ is the $j$-th unit vector, yields:
	\begin{align*}
		\sum_{t=1}^\tA w_t(\mu) &= \sum_{t=1}^\tA S_t \cdot \frac{\bar f}{\underline \rho_{T^*}} e_j^\top (\rho_{T^*} - b_t(x_t))\\
		&=  \frac{\bar f}{\underline \rho_{T^*}} \cdot \left( \sum_{t=1}^\tA S_t \rho_{T^*,j} - \sum_{t=1}^\tA S_t b_{t,j}(x_t) \right)\\
		&\leq  \frac{\bar f}{\underline \rho_{T^*}} \cdot \left( \sum_{t=1}^\tA S_t \rho_{T^*,j} - \sum_{t=1}^\tA b_{t,j}(x_t) \right)\\
		&\leq  \frac{\bar f}{\underline \rho_{T^*}} \cdot \left( \sum_{t=1}^\tA S_t \rho_{T^*,j} + \bar b - T^* \rho_{T^*} \right)\\
		&\leq \frac{\bar f}{\underline \rho_{T^*}}\cdot \left(\bar b - \left\{\sum_{t=1}^{\tau_2} S_t \rho_{T^*,j} - \sum_{t=1}^\tA S_t \rho_{T^*,j} \right\} \right) &\left(T^* = \sum_{t=1}^{\tau_2} S_t \right)\\
		&= \frac{\bar f \bar b}{\underline \rho_{T^*,j}} - \bar f \cdot \sum_{t = \tA + 1}^T\frac{S_t \rho_{T^*}}{\underline \rho_T}\\
		&\leq \frac{\bar f \bar b}{\underline \rho_T} - \sum_{t = \tA + 1}^T S_t \cdot\bar f
	\end{align*}
	Finally, if we put everything together, we get
	\begin{align*}
		\clubsuit \leq \frac{\bar f \bar b}{\underline \rho_{T^*}} + E(\tau_2, \mu) \le \frac{\bar f \bar b}{\underline \rho_{T^*}} + \frac 1 {2\sigma} (\bar{b} + \bar\lambda)^2 \eta \cdot \tau_2 + \frac{1}{\eta} V_h(\mu,\mu_1) \ ,	
	\end{align*}
	where we have used the definition of $E(\tau_2, \mu)$. The theorem follows from observing that all of our choices of $\mu$ in the above discussion lie in the set $\{0, (\bar f/\underline \rho_{T^*}) e_1,\ldots, (\bar f/\underline \rho_{T^*}) e_m\}$.
\end{proof}









